Behind the Scenes: On the Relationship Between Developer Experience and Refactoring

Refactoring is widely recognized as one of the efficient techniques to manage technical debt and maintain a healthy software project through enforcing best design practices or coping with design defects. Previous refactoring surveys have shown that code refactoring activities are mainly executed by developers who have sufficient knowledge of the system's design and disposing of leadership roles in their development teams. However, these surveys were mainly limited to specific projects and companies. In this paper, we explore the generalizability of the previous results by analyzing 800 open-source projects. We mine their refactoring activities, and we identify their corresponding contributors. Then, we associate an experience score to each contributor in order to test various hypotheses related to whether developers with higher scores tend to 1) perform a higher number of refactoring operations 2) exhibit different motivations behind their refactoring, and 3) better document their refactoring activity. We found that (1) although refactoring is not restricted to a subset of developers, those with higher contribution scores tend to perform more refactorings than others; (2) while there is no correlation between experience and motivation behind refactoring, top contributed developers are found to perform a wider variety of refactoring operations, regardless of their complexity; and (3) top contributed developer tend to document less their refactoring activity. Our qualitative analysis of three randomly sampled projects shows that the developers who are responsible for the majority of refactoring activities are typically in advanced positions in their development teams, demonstrating their extensive knowledge of the design of the systems they contribute to.

==> Charts/Distribution_refactoring_operations.tex <==
\begin{figure}[htbp]
\centering
\begin{tikzpicture}
\begin{scope}[scale=0.8]
\pgfplotsset{%
    width=.83\textwidth,
    height=1.5\textwidth
}
\begin{axis}[ 
    xmajorgrids=true,
    xbar, 
    xmin=0,
    xlabel={Percentage (\%)},
    symbolic y coords={{Extract Method}, {Inline Method}, {Rename Method},{Move Method}, {Move Attribute}, {Pull up Method}, {Pull up Attribute}, {Push down Method}, {Push down Attribute},{Extract Superclass}, {Extract Interface}, {Move Class}, {Rename Class},{Change Package}, {Extract Class},{Extract Subclass}, {Extract Variable}, {Inline Variable}, {Parameterize Variable}, {Rename Variable},{Rename Parameter},{Rename Attribute},{Replace Attribute},{Move Source Folder}, {Replace Variable w/ Attribute}, {Move \& Rename Attribute}, {Move \& Rename Class},{Extract \& Move Method}},
    ytick=data,
    legend style={
    	at={(0.3,-0.07)},
        anchor=north,
        legend columns=-1,
        /tikz/every even column/.append style={column sep=0.5cm}
        },
    nodes near coords,
    every node near coord/.append style={font=\tiny},
    nodes near coords align={horizontal},
     enlarge y limits=0.02,
]

% Top 5
\addplot[fill=violet,draw=black!70,tickwidth = 0pt,bar width=4pt,label style={font=\small}, tick label style={font=\small}] coordinates {(6.97,{Extract Method}) (1.09,{Inline Method}) (11.95,{Rename Method}) (5.41,{Move Method}) (6.34,{Move Attribute}) (3.69,{Pull up Method}) (8.96,{Pull up Attribute}) (1.75,{Push down Method}) (0.62,{Push down Attribute}) (7.78,{Extract Superclass}) (0.25,{Extract Interface}) (11.30,{Move Class}) (3.58,{Rename Class}) (0.35,{Change Package}) (1.02,{Extract Class}) (0.15,{Extract Subclass}) (3.01,{Extract Variable}) (0.61,{Inline Variable}) (0.53,{Parameterize Variable}) (11.65,{Rename Variable}) (6.45,{Rename Parameter}) (16.36,{Rename Attribute}) (0.03,{Replace Attribute}) (0.67,{Move Source Folder}) (0.51,{Replace Variable w/ Attribute}) (0.03,{Move \& Rename Attribute}) (1.11,{Move \& Rename Class}) (2.02,{Extract \& Move Method})};

% Rest
\addplot[fill=cyan,draw=black!70,tickwidth = 0pt,bar width=4pt,label style={font=\small}, tick label style={font=\small}] coordinates {(1.66,{Extract Method}) (0.22,{Inline Method}) (5.06,{Rename Method}) (1.22,{Move Method}) (0.72,{Move Attribute}) (0.94,{Pull up Method}) (0.35,{Pull up Attribute}) (0.12,{Push down Method}) (0.04,{Push down Attribute}) (0.13,{Extract Superclass}) (0.02,{Extract Interface}) (1.05,{Move Class}) (0.87,{Rename Class}) (0.05,{Change Package}) (0.22,{Extract Class}) (0.01,{Extract Subclass}) (0.48,{Extract Variable}) (0.04,{Inline Variable}) (0.15,{Parameterize Variable}) (14.31,{Rename Variable}) (2.59,{Rename Parameter}) (68.74,{Rename Attribute}) (0,{Replace Attribute}) (0.05,{Move Source Folder}) (0.04,{Replace Variable w/ Attribute}) (0,{Move \& Rename Attribute}) (0.50,{Move \& Rename Class}) (0.29,{Extract \& Move Method})};
\legend{Top 5 \% of developers, Rest of developers}
\end{axis}
\end{scope}
\end{tikzpicture}

\caption{Distribution of refactoring operations performed by the top 5 \% and the remaining set of developers}
\label{fig:distirbution}
\end{figure}



==> Review.tex <==
----------------------- REVIEW 1 ---------------------
SUBMISSION: 8
TITLE: On the Relationship Between Developer Experience and Refactoring: An Exploratory Study and Preliminary Results
AUTHORS: Eman Abdullah Alomar, Anthony Peruma, Christian Newman, Mohamed Wiem Mkaouer and Ali Ouni

----------- Overall evaluation -----------
SCORE: 1 (weak accept)
----- TEXT:
The authors investigated the relationship between refactoring activities and developers experience by analyzing the DCR values of developers who perform only refactoring and other activities. They also split developers based on their experience scores and then analyzed their refactoring activities. The results reveal that (1) more experienced developers tend to perform refactoring more than others and (2) developers who are responsible for the majority of refactoring activities are on advanced positions in their development teams.

Points in favor:
+ Interesting topic
+ Well-structured and easy to follow

Points against:
- the novelty is low
- unclear research implications based on the investigation results
 
Overall, I think that this paper is very interesting which is well-structured and easy to follow. However, my biggest concern is that novelty is very low for the paper. As mentioned in the papers, the authors replicate previous studies with  800 open source projects. So, the findings are not surprising at all. Furthermore, Section 3.3 focuses on future directions only. So I could not understand research implications based on the investigation results. I think that the authors should compare the distribution of DCR values in this paper and their previous work [19]

Finally, Section 3.1 says that "As shown in Figure 2, we looked at two types of distributions - developers that only performed refactoring operations, and developers that performed a mix of refactoring and non-refactoring operations on the source code".  But I could not understand Figure 2. Does the "All Commits" represent the distribution of  DCR values for developers that only performed refactoring operations? For me, "All Commits" seems that these commits contain not only refactoring activities but also non-refactoring activities. 



----------------------- REVIEW 2 ---------------------
SUBMISSION: 8
TITLE: On the Relationship Between Developer Experience and Refactoring: An Exploratory Study and Preliminary Results
AUTHORS: Eman Abdullah Alomar, Anthony Peruma, Christian Newman, Mohamed Wiem Mkaouer and Ali Ouni

----------- Overall evaluation -----------
SCORE: 2 (accept)
----- TEXT:
This paper presents an empirical study that explores the generalizability of previous empirical results on developers' refactoring activities by analyzing 800 open-source projects. The focus of the study is the hypothesis of whether developers with higher scores tend to perform a higher number of refactoring operations. The results show that (1) developers with higher experience scores tend to perform more refactorings; (2) developers who are responsible for the majority of refactoring activities are typically on advanced positions in their development
teams.

I think this paper is interesting. The investigation of the relationship between refactoring activities and developer experiences is important to understand the practice of refactoring. The study involves both quantitative and qualitative analysis. The paper is well written and easy to follow.

My concerns about the paper are listed below.
1) The scores used to measure the experience of developers may not well reflect the real developer experience.
2) The findings of the study are of no surprise. It is better to provide more insights for further research and practice.
